Referee: Reference-Free Sentence Summarization with Sharper Controllability through Symbolic Knowledge Distillation

We present Referee, a novel framework for sentence summarization that can be trained reference-free (i.e., requiring no gold summaries for supervision), while allowing direct control for compression ratio. Our work is the first to demonstrate that reference-free, controlled sentence summarization is feasible via the conceptual framework of Symbolic Knowledge Distillation (West et al., 2022), where latent knowledge in pre-trained language models is distilled via explicit examples sampled from the teacher models, further purified with three types of filters: length, fidelity, and Information Bottleneck. Moreover, we uniquely propose iterative distillation of knowledge, where student models from the previous iteration of distillation serve as teacher models in the next iteration. Starting off from a relatively modest set of GPT3-generated summaries, we demonstrate how iterative knowledge distillation can lead to considerably smaller, but better summarizers with sharper controllability. A useful by-product of this iterative distillation process is a high-quality dataset of sentence-summary pairs with varying degrees of compression ratios. Empirical results demonstrate that the final student models vastly outperform the much larger GPT3-Instruct model in terms of the controllability of compression ratios, without compromising the quality of resulting summarization.

==> graveyard/old_intro.tex <==
\section{Introduction}

% We present referee... vast majority of prior work ss assumes sentences are given . HOwever, recent work XYZ show they dont work as well for new domains. Therefore recent work emphasized
% our work is the first to demonstrate... SKD
% one key benefit/byprodyct of our method is that we can directly incorporate length control by design which no one modeled explicitly, maybe as posthoc filter? this vastly contrast with how humans summarize, they can flexibly reduce compression ratio. 
% now iterative SKD
% 



% One of our key-contributions is a simple and effective mechanism for length control, prev work either did not model length control as part of a summ model, or either (...). However, prior work also demonstrated not being able to control length [larger ]

% Novelties: length-control; kd for summarization; new use of IB principle starting with non-contextual summaries (enhancing refree summarization); maybe iteration?

% Paragraph of knowledge distillation itself: although some recent work has explore in kd context, we are the first to adapt that for summ. Mix from guidance from GPT3 instruct and kdistill.

Neural network-based approaches have improved text summarization significantly \citep{rush2015neural, nallapati-etal-2016-abstractive}. However, these methods are successful because they leverage large-scale text-summary paired datasets to train supervised models. These datasets are costly to create, and naturally-occurring summarization datasets (such as news highlights) are noisy and not easily found in many domains. This motivates the need for developing unsupervised or self-supervised models for summarization. In this area, autoencoder approaches are well-known \citep{miao2016language,baziotis-etal-2019-seq}, as well as information-bottleneck principle inspired heuristics \citep{west-etal-2019-bottlesum}.% BottleSumEx is an extractive sentence summarization heuristic that keeps only the information relevant to predict the immediate next sentence. Like many extractive sentence summarizers, BottleSumEx suffers from disfluencies and often removes crucial components like the main verb.% To mitigate this, the authors feed these noisy sentence summarizations as training data to a pretrained transformer, to create BottleSumSelf. Unfortunately, context is not fed to BottleSumSelf, losing the information-bottleneck principled approach. % Recently, \citep{} has shown that using the token \texttt{TL;DR} after a sentence encourages GPT2 to summarize the sentence.

Recently, large language models like GPT3 have shown some few-shot summarization capability, outputting fluent sentence summaries when prompted with few high-quality examples. Nonetheless, they still have some of the known problems of abstractive summarizers, such as hallucinating. Moreover, often GPT3 does not compress the input at all (see \S\ref{sec:analyze-gpt3}).

% highlighting too much GPTx
% no equation, or modeling component (it looks like corpus)
% length control, all components should be there. Look a symbolic kd paper fig1.

\input{figures/fig_1}

%\begin{figure}[t]
%    \centering
%    \includegraphics[width=\linewidth]{Schema.png}
%    \includegraphics[width=\linewidth]{Schema.png}
%    \caption{Depiction of the iterative procedure to produce shorter and better summaries. \texttt{FILTER} is an automatic function that will discard some sentence+summary pairs that are not deemed of enough quality. The kept sentence pairs will be the only ones used for training. \ms{maybe not the right place}}
%    \label{fig1}
%\end{figure}

Sentence summarization is a smaller-scale version of document summarization, but many of the same issues arise: lack of faithfulness, bad information selection. Sentence summarization improvements also impact related tasks like text simplification and compression \citep{schumann2020discrete}. Summarizing at the sentence level also allows for leveraging other systems, like Natural Language Inference (NLI).

%\ms{Missing motivation for length-controlled summaries}
Sentence summaries may be appropriate or not depending on context and the needs of each user. \yejin{this previous sentence is LOL... i think this sentence is great to include in the Limitation section, but not in the intro, and certainly not as an opening sentence of *any* paragraph of an intro :)} Nonetheless, attributes like the summary length are mostly treated as an attribute of each model, and not a variable to control for \cite{tbd}. Controlling for summary length has become increasingly important, since several applications --like tweets, and text boxes in general-- force an upper limit on character length. Moreover, reliable sentence summarization datasets are scarce, and it is difficult to effectively train supervised models when lacking reference summaries showcasing desired behaviors. \yejin{i don't think we need an entire paragraph dedicating to pitch the importance of the length control, and even if we were to, it should appear *after* we pitch what we do first, in order to maintain tension/excitement toward our paper (we lose interests from readers if we talk too long about what others did or did not do well previously...) }

\yejin{the description of what we do, and what aspects of it are novel, appears too late in the intro, and not informative enough; i think we need to play up the knowledge distillation angle, and how iterative KD is the first, and with filters we can enhance the quality dramatically should be better highlighted}

In this work, we show that starting from automatically-generated, fluent, lightly-compressed sentence summaries, we can create a model --\firstphasemodelname{}-- that outputs better and more succinct summaries. % than the ones it was trained on.
We achieve this by iteratively fine-tuning a GPT2 Large model, effectively distilling knowledge from GPT3.
Each intermediate iteration serves as a data generator for a another model, \secondphasemodelname{}, that can control for sentence summary length by separating the space of possible summary compression ratios into 10 equally-distributed categorical variables.

%We start by filtering a GPT3-generated sentence summarization dataset, only retaining the high quality and short summaries, and fine-tuning a GPT2 Large model with that data. Then, in each successive iteration we generate summaries from the fine-tuned GPT2 Large model, filter for quality and summary length more aggresively, and then fine-tune further using the newly-generated data. This effectively distills knowledge from GPT3 onto a smaller model. Besides distillation, this allows the resulting model to show behaviors that the initial dataset did not have examples for, such as compressing more than any original training example.

\yejin{once intro is strongly crafted, we usually do not need (or want) to have a bullet list of contributions...}

Our contributions are as follows:
% Key novelties of our work include the ability of controlling to compress sentences at any compression ratio range; the usage of knowledge distillation from LLMs in the context of summarization; and the ability to create contextual sentence summaries using the Information Bottleneck principle, even if initial summaries are not contextually aware. \modelname{} performs on par with the initial LLMs in terms of hallucination and information preservation, and outperforms GPT3 for shorter summaries, while providing control for length

\begin{itemize}
    \item We propose an approach, \firstphasemodelname{}, that iteratively distills symbolic knowledge from automatically-generated sentence summaries. In each iteration, the previous iteration's student serves as teacher. GPT3 is used as the kickstarter of our iterative process, and all later iterations are self training.% Our approach allows to flexibly promote any binary condition in summaries, which we demonstrate through 
    \item We develop \secondphasemodelname{}, a model that can reliably control for the desired level of sentence summary compression. Length control is fine-grained, allowing the user to requests compression ratios in increments of 10\%. % We show that we can request any compression ratio range $[0.1k, \ 0.1(k +1)]$ with $k \in \{0,\cdots,9\}$ and the output will fall in that range with up to \ms{88}\% of the time. 
    \item As a by-product of generating sentence summarization data for each intermediate iteration of \firstphasemodelname{}, we release an automatically-generated sentence summarization dataset of \ms{100k?, but I can make infinitely many}.
    \item We show a way of contextualizing sentence summaries in \firstphasemodelname{} by leveraging the information bottleneck principle. In contrast with prior work, our approach does not require that initial summaries are constructed using this principle.
    %\item Our approach allows to flexibly promote any binary condition in summaries. We demonstrate that through iterait selecting for shorter summary lengths, we can develop a model that generates significantly shorter summaries than the ones originally trained on.
    %\item Through iterative filtering, we introduce a contextual sentence summarization model, based on the Information Bottleneck principle.
    %\item Thanks to the newly introduced capabilities of generating data at any length, we develop a model that can reliably summarize at any compression ratio. 
\end{itemize}


==> graveyard/older_abstracts.tex <==
\begin{abstract}
%\ms{Version written on June 14th}

\ms{Yejin's hunch: start directly by our contribution}
\ms{Yejin: Self supervised summarization through the lens of knowledge distillation}
\ms{Key conceptual novelties work are three-fold: ..., we adapt iterative-learning, length-controlled summarization.}

Large language models (LLMs) often show good few-shot sentence summarization capabilities, which is especially useful for domains lacking reference summaries. Nonetheless, LLMs sometimes hallucinate, and it is difficult to control them to generate summaries with specific length or compression rate. Length-controlled summarization has become increasingly important, as many applications (like tweets) have a strict character upper bound.

In this work, we propose \modelname{}, a continual-learning approach to distill knowledge from GPT3 sentence summaries onto significantly smaller models while also encouraging any desired binary condition. \modelname{} consists of two key components. First, \firstphasemodelname{} can iteratively select for any condition throughout training, such as compressing aggressively, or generating contextually aware summaries. This results in a diverse and high-quality set of sentence summaries. We then use this initial data set to train a length-controlled sentence summarization model (\secondphasemodelname{}) that can summarize at any compression range, even when GPT3 did not originally generated any summary at that compression rate. \modelname{} performs on par to the initial sentence summaries, and often outperforms GPT3 for shorter summaries, while providing control for length.
\end{abstract}

\begin{abstract}
\ms{Version written on June 16th, 1am PDT, convincing people about control}

Sentence summaries may be appropriate or not depending on context and the needs of each user. Nonetheless, controllable sentence summarization generation is understudied in the literature. Moreover, reliable sentence summarization datasets are scarce, and it is difficult to effectively train supervised models when lacking reference summaries showcasing desired behaviors.
In this work, we propose \modelname{}, a continual-learning approach that distills sentence summarization knowledge from Large Language Models (LLMs) onto significantly smaller ones, while also encouraging any measurable binary conditions. \modelname{} does not require any reference summaries, but can still outperform supervised baselines for our task. Key novelties of our work include the ability of controlling to compress sentences at any compression ratio range; the usage of knowledge distillation from LLMs in the context of summarization; and the ability to create contextual sentence summaries using the Information Bottleneck principle, even if initial summaries are not contextually aware. \modelname{} performs on par with the initial LLMs in terms of hallucination and information preservation, and outperforms GPT3 for shorter summaries, while providing control for length.

%No two summaries are created equal. Depending on context and the needs of each user, different summaries may be the most suitable. For example, controlling for length has become increasingly important, as many applications (like tweets) have a strict character upper bound. Users may also want to generate summaries that take context into account.
%Large language models (LLMs) can generate sentence summaries using few-shot prompting, which is especially useful for domains lacking reference summaries. Nonetheless, LLMs sometimes hallucinate, and it is difficult to control them to generate summaries with desired behaviors like compression ratio. Length-controlled summarization has become increasingly important, as many applications (like tweets) have a strict character upper bound.

\end{abstract}

\begin{abstract}
%\ms{Version written on June 16th, 2pm PDT}
%We propose \modelname{}, a continual-learning method for sentence summarization that is both reference free and deliberately controlled. [[we use gpt3, applied anywhere, without little control. we get the best of both worlds by distilling quality gpt3's but also notions of control that are up to the user]] To design our method, we take advantage of existing large language models like GPT-3, which can generate summaries without any reference but offer little control or [knowledge distillation]

%In this work, we propose \modelname{}, a continual-learning approach that distills sentence summarization knowledge from Large Language Models (LLMs) onto significantly smaller ones, while also encouraging any measurable binary conditions. \modelname{} does not require any reference summaries, but can still outperform supervised baselines for our task. Key novelties of our work include the ability of controlling to compress sentences at any compression ratio range; the usage of knowledge distillation from LLMs in the context of summarization; and the ability to create contextual sentence summaries using the Information Bottleneck principle, even if initial summaries are not contextually aware. \modelname{} performs on par with the initial LLMs in terms of hallucination and information preservation, and outperforms GPT3 for shorter summaries, while providing control for length.

\sk{Abstract Suggestion}

We present \modelname{}, a nearly unsupervised method for controllable sentence summarization. Leveraging few-shot inference capabilities of large language models such as GPT3, we first synthesize a small summarization corpus. We then bootstrap this corpus by iteratively self-training a significantly smaller model by (1) learning a noisy model on the synthetic dataset, and (2) synthesizing additional data by summarizing more sentences using this model and filtering out the noise. Deploying filters based on output length, and contextual coherence (like NLI and next sentence prediction (or information bottleneck?)), we create a high-quality dataset of ${\sim}$100K sentence-summary pairs with diverse compression ratios (ranging from 80-90\% to 10-20\%). Finally, we show that a summarization model trained using this dataset vastly outperforms a much larger GPT3 model in terms of length control without compromising on information preservation and fluency.
\end{abstract}

\begin{abstract}
\ms{Melanie after reading Sachin's suggestion} 

We present \modelname{}, a knowledge-distillation model for sentence summarization that both does not require any reference summaries and is deliberately controlled. We specifically explore controlling for summary length, as well as generating contextual summaries by leveraging the Information Bottleneck principle. We also control for summary factuality by using a pre-trained Natural Language Inference model. \modelname{} is iteratively-trained to progressively select for desired behaviors that may not occur in the initial data. At each iteration, we filter the synthetically-generated input data, train from it, and generate another synthetic corpus that the next iteration will use as training data. We leverage few-shot inference capabilities of large language models (LLMs) by using GPT3 sentence summaries as the initial data in our distillation procedure. Throughout our iterative filtering, we can distill knowledge from GPT3 onto significantly smaller models while also overcoming the little control LLMs offer for customizing summaries.
Intermediate datasets from this iterative model result in a high-quality dataset of $\sim$100K sentence-summary pairs with more diversity of compression ratios (ranging from 10\% to 100\%) than the original GPT3 summaries. Finally, we show that a sentence summarization model trained using this diverse dataset vastly outperforms a much larger GPT3 model in terms of length control without compromising on information preservation and factuality.
\end{abstract}


